Robust Edge-Preserved Surface Mesh Polycube Deformation

The problem of polycube construction or deformation is an essential problem in computer graphics. In this paper, we present a robust, simple, efficient and automatic algorithm to deform the meshes of arbitrary shapes into their polycube ones. We derive a clear relationship between a mesh and its corresponding polycube shape. Our algorithm is edge-preserved, and works on surface meshes with or without boundaries. Our algorithm outperforms previous ones in speed, robustness, efficiency. Our method is simple to implement. To demonstrate the robustness and effectiveness of our method, we apply it to hundreds of models of varying complexity and topology. We demonstrat that our method compares favorably to other state-of-the-art polycube deformation methods.

==> comparison.tex <==
\section{Comparison and Evaluation} 
To evaluation and compare out method with other automatic methods in \cite{Livesu:2013:PolyCut}. We propose to measure the distortion by the stretching energy proposed in  \cite{Hui:2016:Deform,Liu:2008:PQT,Chao:2010:SGM}.  The  stretching energy between two surfaces is an measurement of the deformation of surfaces in 3 dimensions \cite{Hui:2016:Deform}. 
This energy measures the quantity
 \begin{equation}
 \int_{s} 
 (\sigma_1(p) -1)^2 + (\sigma_2(p)-1)^2
 \;\; dA_{g}(p) 
 \end{equation}
 where $\sigma_1(p)$ and  $\sigma_2(p)$ are the
 the maximum and (resp.) minimal stretching ratios.  The energy is defined as:
 
 \begin{align} 
 E_(S,P)   =\sum_{he_{vw}} \cot (a_{vw})
 \| (\bb{x}^{\prime}_{v}-\bb{x}^{\prime}_{w} )-R(t_{vw})(\bb{x}_{v}-\bb{x}_{w})\|^{2} 
 \label{func:StretchingEnergy}
 \end{align}
 where $\|\cdot\|^2$ is the standard 3-vector norm.
 In above, 
 the symbol $he_{vw}$ represents the half edge from
 the vertex $v$ to $w$, and
the sum is over all the
 half edges of the mesh.
 The symbol $a_{vw}$ is the angle of the 
 corner opposite to the half edge $he_{vw}$ in its triangle.
 $R(t_{vw})$ is the $3 \times 3$ (variable) rotation matrix associated with the
 triangle face associated with the half edge $he_{vw}$.
 
 The stretching energy $E(S,P)$ measures only stretching , to measure the shrinking, we use the energy $E(P,S)$. With both of them together, we measures the following quantity:
 
  \begin{equation}
  \int_{s} 
  (\sigma_1(p) -1)^2 + (\sigma_2(p)-1)^2+(\frac{1}{\sigma_1(p)} -1)^2 + (\frac{1}{\sigma_2(p)}-1)^2
  \;\; dA_{g}(p) 
  \end{equation}
 
 
 
 
 
 
 
 

 
  
 
 
